SABLE: Secure And Byzantine robust LEarning

Due to the widespread availability of data, machine learning (ML) algorithms are increasingly being implemented in distributed topologies, wherein various nodes collaborate to train ML models via the coordination of a central server. However, distributed learning approaches face significant vulnerabilities, primarily stemming from two potential threats. Firstly, the presence of Byzantine nodes poses a risk of corrupting the learning process by transmitting inaccurate information to the server. Secondly, a curious server may compromise the privacy of individual nodes, sometimes reconstructing the entirety of the nodes' data. Homomorphic encryption (HE) has emerged as a leading security measure to preserve privacy in distributed learning under non-Byzantine scenarios. However, the extensive computational demands of HE, particularly for high-dimensional ML models, have deterred attempts to design purely homomorphic operators for non-linear robust aggregators. This paper introduces SABLE, the first homomorphic and Byzantine robust distributed learning algorithm. SABLE leverages HTS, a novel and efficient homomorphic operator implementing the prominent coordinate-wise trimmed mean robust aggregator. Designing HTS enables us to implement HMED, a novel homomorphic median aggregator. Extensive experiments on standard ML tasks demonstrate that SABLE achieves practical execution times while maintaining an ML accuracy comparable to its non-private counterpart.

==> app_hts.tex <==
\section{HTS: implementation details}\label{subsec:app_hts}
\textbf{Terminology, conventions, and assumptions.}
All operators on vectors of slots that will be used throughout are
homomorphic and operate slot-wise.

We recall that the typical slot in a generic vector \vslots\ is a
polynomial whose coefficients record the digits of an integer
represented in its base-$B$ expansion as in
\eqref{eq:integer.digit.decomposition}.
The digits can be individually recorded into new vectors of
slots thanks to the digit extraction operators, $\extract_i$ for $i=0,\,\dots,\,N$,
see \eqref{def:digit.extraction}.
As a matter of terminology,
\defn{constant polynomial vectors of slots}
is a vector all of whose slots are represented by constant
polynomials.

In Section~\ref{sec:operators.on.digits} we introduce auxiliary
homomorphic operators which will in practice only be applied to vectors of
slots resulting from digit extraction, 
hence the subscript `\texttt{digit}' in the notation and the use of
\texttt{d} and \texttt{d}' instead of \vslots\ and \vslots'.
Note that they are nevertheless well defined for arbitrary vectors.
We stress that all operators in Section~\ref{sec:operators.on.digits}
are well defined for arbitray vectors of slots, but that the notation
\texttt{d} and \texttt{d'} simply recalls that they are meant to be
used on constant polynomial vectors of slots.
In Section~\ref{subsec:homomorphic.comparison.operators}, via the
lexicographic order we combine such
auxiliary operators to construct operators on vectors whose slots
contain in their coefficients the digits of integers expanded with
respect to a known base $B$ as in \eqref{eq:integer.digit.decomposition}.
Finally in Section~\ref{subsec:hts_algo}, building upon these
operators we introduce our Homomorphic Trimmed Sum operator
\trimmedsum.

\subsection{Auxiliary homomorphic operators}\label{sec:operators.on.digits}
We define the function $\1$ on boolean values by 
\begin{equation}
  \1\left(\texttt{true}\right)=0,\qquad
  \1\left(\texttt{false}\right)=1
\end{equation}
\smallskip

\textbf{Equality test on constant polynomial vectors.}
If $k$ is an integer,
then the equality test function
$\1(c==k)$ on the variable $c$ restricted to the range $\{M_1,\,\dots,\,M_2\}$
can be implemented via an interpolation polynomial 
$\textrm{Pol}_{\texttt{Eq},\,k,\,M_1,\,\dots,\,M_2}$:
\begin{equation}
  \1(c==k) = \textrm{Pol}_{\texttt{Eq},\,k,\,M_1,\,M_2}(c),
  \qquad c\in \{M_1,\,\dots,\,M_2\}
  \end{equation}
We define the homomorphic slot-wise operator with
\begin{equation}
  \texttt{Eq}[\texttt{d},\,k;\,M_1,\,M_2]
  := \textrm{Pol}_{\texttt{Eq},\,k,\,M_1,\,M_2}[\texttt{d}]
\end{equation}
which we emphasize is meant slot-wise, i.e. operating on each slot of
the vector \texttt{d}.
When \texttt{d}\ is a vector all of whose slots are constant
polynomials with value in the range $\{M_1,\,\dots,\,M_2\}$,
$\texttt{Eq}[\texttt{d};\,k,\,M_1,\,M_2]$ is a vector all of whose slots
are constant polynomials,
with constant coefficient equal to `\texttt{1}' if the value of the
corresponding slot equals $k$ and `\texttt{0}' otherwise.

\textbf{Zero test on constant polynomial vectors.}
For $k=0$ we set
\begin{equation}
  \texttt{Zero}[\texttt{d};\,M_1,\,M_2] := \texttt{Eq}[\texttt{d},\,0;\,M_1,\,M_2]
\end{equation}

\textbf{Negativity test on constant polynomial vectors.}
The negativity test over the range $\{M_1,\,\dots,\,M_2\}$ can be implemented
via the polynomial
\begin{equation}
  \textrm{Pol}_{\texttt{Neg},\,M_1,\,M_2} :=
  \sum\limits_{k=M_1, k<0}^{M_2}\textrm{Pol}_{\texttt{Eq},\,k,\,M_1,\,M_2}
\end{equation}
since
$\1(c<0) = \textrm{Pol}_{\texttt{Neg},\,M_1,\,M_2}(c)$
for $c\in\{M_1,\,\dots,\,M_2\}$.
In turn, this polynomial yields a slot-wise homomorphic operator
\begin{equation}
  \texttt{Neg}[\texttt{d};\,M_1,\,M_2] := \textrm{Pol}_{\texttt{Neg},\,M_1,\,M_2}[\texttt{d}]
\end{equation}
again meant slot-wise.
When \texttt{d}\ is a vector all of whose slots are constant
polynomials with value in the range $\{M_1,\,\dots,\,M_2\}$,
$\texttt{Neg}[\texttt{d};\,M_1,\,M_2]$ is a vector all of whose slots
are constant polynomials, 
with constant coefficient equal to `\texttt{1}' if the constant value of the
corresponding slot is negative and `\texttt{0}' otherwise.

\textbf{Membership test on constant polynomial vectors}
Given two integers $\underline r\le \overline r$, 
the polynomial
\begin{equation}
  \textrm{Pol}_{\texttt{Btw},\,\underline r,\,\overline r,\,M_1,\,M_2} :=
  \sum\limits_{k=M_1, k<0}^{M_2}\textrm{Pol}_{\texttt{Eq},\,k,\,M_1,\,M_2}
\end{equation}
yields a slot-wise homomorphic operator
\begin{equation}
  \texttt{Btw}[\texttt{d},\,\underline r,\,\overline r;\,M_1,\,M_2]
  := \textrm{Pol}_{\texttt{Btw},\,\underline r,\,\overline r,\,M_1,\,M_2}[\texttt{d}]
  \label{def:between.operator}
\end{equation}
again meant slot-wise.
When \texttt{d}\ is a vector all of whose slots are constant
polynomials with value in the range $\{M_1,\,\dots,\,M_2\}$,
$\texttt{Btw}[\texttt{d};\,\underline r,\,\overline r,\,M_1,\,M_2]$ is a vector all of whose slots
are constant polynomials, 
with constant coefficient equal to `\texttt{1}' if the constant value of the
corresponding slot is in the range $[\underline r,\,\overline r]$ and
`\texttt{0}' otherwise.

\textbf{Comparison of constant polynomial vectors.}
We introduce two operators which will be used on vectors of slots
after digit extraction.

We define a slot-wise homomorphic operator on two vectors of slots,
parametrized by an integer $M$, with
\begin{equation}
  \texttt{LT}_\texttt{digit}[\texttt{d},\,\texttt{d}';\,M] := \texttt{Neg}[\texttt{d}-\texttt{d}';\,-M,\,M]
\end{equation}
When \texttt{d}\ and \texttt{d}'\ are two constant polynomial vectors, all
of whose constant values are in the range $[0,\,M]$,
$\texttt{LT}_\texttt{digit}[\texttt{d},\,\texttt{d}';\,M]$ returns a constant polynomial
vector,
with a `\texttt{1}' if the corresponding slot of \texttt{d}\ is less than that of
\texttt{d}',
and a `\texttt{0}' otherwise.

Similarly, 
we define a slot-wise homomorphic operator on two vectors of slots,
parametrized by an integer $M$, with
\begin{equation}
  \texttt{Eq}_\texttt{digit}[\texttt{d},\,\texttt{d}';\,M] := \texttt{Eq}[\texttt{d}-\texttt{d}';\,-M,\,M]
\end{equation}
When \texttt{d}\ and \texttt{d}'\ are two constant polynomial vectors, all
of whose constant values are in the range $[0,\,M]$,
$\texttt{Eq}_\texttt{digit}[\texttt{d},\,\texttt{d}';\,M]$ returns a constant polynomial vector,
with a `\texttt{1}' if the corresponding slot of \texttt{d}\ equals that of
\texttt{d}', and a `\texttt{0}' otherwise.

\subsection{Homomorphic Comparison Operators}
\label{subsec:homomorphic.comparison.operators}
\textbf{The less-than operator \texttt{LT}.}
Integers $a\,=\,\sum_{i=0}^{\ordp-1}c_iB^i$ and  $a'\,=\,\sum_{i=0}^{\ordp-1}c_i'B^i$ decomposed according to \eqref{eq:integer.digit.decomposition} can be ordered via the lexicographic ordering on their digits with the formula
\begin{equation}
  \1\left(a<a'\right) \,=\, 
  \sum_{i=0}^{\ordp-1} \Big(\1\left(c_i<c_i'\right)
  \times\prod_{j=i+1}^{\ordp-1}
  \1\left(c_j==c_j'\right) \Big)
  %\label{eq:LT.lexicographic}
\end{equation}
Taking our cue from this identity, we introduce our \defn{less-than}
operator on vectors of slots as
\begin{align}
  \texttt{LT}[\vslots,\,\vslots';\,B] 
  := \,&
  \sum_{i=0}^{\ordp-1} \Big(
  \texttt{Neg}[\texttt{d}_i-\texttt{d}_i;\,-B,\,B]
  %\label{eq:homomorphic.LT}
  \\
  &\quad
  \times\prod_{j=i+1}^{\ordp-1}
  \texttt{Zero}[\texttt{d}_j-\texttt{d}'_j;\,-B,\,B]
  \Big)
  \notag
\end{align}
where
$\texttt{d}_i := \extract_i[\vslots]$ and
$\texttt{d}'_i:=\extract_i[\vslots']$
for $i=0,\,\dots,\,N-1$.
By construction, this operator is homomorphic and operates slot-wise.
If the slots stored in \vslots\ and \vslots' represent integers in
their base-$B$ expansion, then $\texttt{LT}[\vslots,\,\vslots';\,B]$
is a constant polynomial vector,
and in each slot, the constant coefficient is a `\texttt{1}` if the
integer represented by the corresponding slot in \vslots\ is less than
that in \vslots', and a `\texttt{0}` otherwise.

\textbf{The rank operator $\rank$.}
Given an ordered list of integer values $a_0, \dots, a_{n-1}$,
we wish to compute their respective ranks
$\textrm{rk}_0,\,\dots,\,\textrm{rk}_{n-1}$ in the list,
namely a reordering of the range $\{0,\,\dots,\,n-1\}$ satisfying
\begin{equation}
  \left\{
  \begin{aligned}
    \textrm{rk}_i<\textrm{rk}_j   \quad & \textrm{if}\quad a_i<a_j\,,\\
    \textrm{rk}_i\ne\textrm{rk}_j \quad &\textrm{if}\quad
    a_i\,==\,a_j\quad \textrm{and}\quad i\ne j\,.
  \end{aligned}
  \right.
  %\label{eq:rank.properties}
\end{equation}
This echoes \eqref{eq:coordinate-wise.sorted}.
For each $i$, the sum $\sum_{j=0}^{n-1}\1(a_i<a_j)$ returns
$\textrm{rk}_i$ only if the value $a_i$ does not repeat in the list.
Following a device from \cite{CetinEtAl}, this issue can be overcome
by taking instead
\begin{equation}
  \textrm{rk}_i := \sum_{k\le i}\1(a_k<a_i) + \sum_{k>i}\1(a_k\le a_i)
\end{equation}
\begin{proof}
    From the definition we see that $0\le \rank_i\le n-1$ for all $i$.
%% We wish to show that $\rank_i\ne\rank_j$ for $i\ne j$ so that the $\rank_i$'s are a reordering of the indices $i=0$ through $n-1$.
Fix now $i\ne j$.
In case $a_i<a_j$,
$\{i\} \cup \left\{k\colon a_k<a_i\right\}\subseteq
\left\{k\colon a_k<a_j\right\}$
so that
\begin{align}
  \textrm{rk}_i
  & = \sum_{k=0}^{n-1} \1(a_i<a_k)
  + \sum_{k=i+1}^{n-1} \1(a_i == a_k) \notag\\
  & < \sum_{k=0}^{n-1} \1(a_k<a_j) \notag \\
  & \le \sum_{k=0}^{n-1} \1(a_k<a_j)
  + \sum_{k=i+1}^{n-1} \1(a_k == a_j) \notag\\
  & = \textrm{rk}_j
\end{align}
and in case $a_i = a_j$, then
$\left\{k\colon\,a_k\,==\,a_i\right\}\,\subsetneq\,\left\{k\colon\,a_k\,==\,a_j\right\}$
and we find similarly that
$\textrm{rk}_i\,<\,\textrm{rk}_j$.
\end{proof}

In order to implement this idea when constructing the \rank\ operator on
vectors of slots, we introduce the auxiliary operator
\begin{equation}
  \texttt{Comp}\left(\vslots,\,\vslots',\,\texttt{b};\,B\right)
  \,=\,
  \left\{
  \begin{array}{rl}
    \lessthan[\vslots,\,\vslots';\,B]&\textrm{if}\quad \texttt{b}\\
    1-\lessthan[\vslots',\,\vslots;\,B]&\textrm{if}\quad \texttt{not b}
  \end{array}
  \right.
  %\label{eq:comp}
\end{equation}
where $\texttt{b}\in\{\texttt{true},\,\texttt{false}\}$.

We now turn to the \rank\ operator on an ordered list of vectors of
slots
$\vslots_0,\,\dots,\,\vslots_{n-1}$.
It is defined as
\begin{equation}
    %\label{eq:rk}
    \rank[
      \{\vslots_j\}_{j=0}^{n-1},\,i;\,B
    ] 
    \,:=\, \sum_{j=0}^{n-1} 
    \texttt{Comp}[\vslots_i,\,\vslots_j,\,\1(i<j);\,B]
\end{equation}
This operator is homomorphic and operates slot-wise.
If the slots in the vectors in the list $\{\vslots_j\}_{j=0}^{n-1}$
represent integers in their base-$B$ expansion,
$\rank[\{\vslots_j\}_{j=0}^{n-1},\,i;\,B]$ is a constant polynomial
vector
where the slot of index $k$ has constant coefficient equal 
to the rank (in the sense of \eqref{eq:rank.properties})
of the integer value represented by the $k$-th slot in the $i$-th
vector $\vslots_i$, within the list of the $k$-th slot
of all the vectors $\vslots_j$, $j=0,\,\dots,\,n-1$.

\subsection{The \aggregator{} Operator}\label{subsec:hts_algo}
Echoing \eqref{eq:cwtm}, our homomorphic trimmed sum operator is
defined as
\begin{align}
  %\label{eq:trimmed_sum}
  &\trimmedsum[\{\vslots_j\}_{j=0}^{n-1};\,f,\,B)\\
    &\quad\quad :=\sum_{i=0}^{n-1}
    \btwn[\texttt{rk}_i,\,f,\,n-f-1;\,0,\,n-1]\vslots_i 
    \end{align}
where \btwn\ is defined in \eqref{def:between.operator}
and where we use the short-hand notation
\begin{equation}
  \textrm{rk}_i := \rank[\{\vslots_j\}_{j=0}^{n-1},\,i;\,B]
\end{equation}
This operator is homomorphic and operates slot-wise.
If the slots in the vectors in the list $\{\vslots_j\}_{j=0}^{n-1}$
represent integers in their base-$B$ expansion,
then $\trimmedsum[\{\vslots_j\}_{j=0}^{n-1},\,f;\,B]$
is a vector containing in its slot of index $k$
the sum of the slots of rank between $f$ and $n-f-1$ among the slots
of index $k$ over the list of vectors $\vslots_j$, for $j=0,\,\dots,\,n-1$.

The homomorphic median operator is a special case of \trimmedsum{}
where only the value with rank $\lfloor\nicefrac{n}{2}\rfloor$ is
selected:
\begin{align}
  %\label{eq:median}
  \median[\{\vslots_j\}_{j=0}^{n-1}\}]
  \,=\,
  \trimmedsum[\{\vslots_j\}_{j=0}^{n-1};\,\lfloor n/2\rfloor,\,B)]
\end{align}

\subsection{Complexity and multiplicative depth}
$\spadesuit$ \textbf{TODO}
explain prohibitive cost of previous comparison operators for large
integers, necessity of base-$B$ expansion and via lexicographic ordering.

Looking at~\eqref{eq:rk},\,\eqref{eq:trimmed_sum}, this algorithm is
quadratic in complexity in the number of inputs $n$.

We note that existing solutions from the literature could have
alternatively been used to build homomorphic implementations of the
less-than, comp, and rank operations.  Yet, we have argued that our
method offers improved performance and this is amply illustrated and
discussed in Section~\ref{subsec:comparison-with-IZ}. In contrast,
the coordinate-wise trimmed sum operation, namely the sum in the
right-hand side of \eqref{eq:cwtm}, is out of reach for existing
solutions prior to our work as already argued in
Section~\ref{subsec:plaintext.encoding.schemes}. %%\ref{subsec:extra.degree.of.freedom}.

The impact of decoupling $B$ from $p$ becomes clearer from the
structure of our operators \zero\ and \negative. While previous work
(e.g.,~ \cite{TanEtAl,IZ21}) uses polynomials of degree $p-1$, here
\zero\ and \negative\ are implemented as polynomials of degree
$2B-1$. The complexity and multiplicative depth of these operators
alone can be significantly reduced by lowering $B$.

Since the complexity and multiplicative depth of 
%% $\btwn(\cdot; f, n-f-1)$ 
\btwn\
are independent of $f$, \trimmedsum\, and \median\, have equal complexities and multiplicative depths.

\subsection{Performance of \trimmedsum{}}\label{subsec:comparison-with-IZ}
This section illustrates the gain in performance when using our method for the task of homomorphic sorting compared to the current state-of-the-art algorithm~\cite{IZ21}, see Table~\ref{table:comparison-with-IZ}. Experiments are run on the same machine.~\footnote{Machine with a 12th Gen Intel© Core™ i7-12700H processor with 62.5GiB memory using a single core.}
For the purpose of illustration, we have chosen to present evaluations of coordinate-wise sorting over $n=4$ vectors with $8$-bit coordinates and dimension $d=9352$ and $5764$.  This choice of values is justified below. In every setting, $q$ is optimized to be as small as possible while still ensuring correctness.
The security level is evaluated in bits and obtained using the latest commit of the lattice estimator~\footnote{\url{https://lattice-estimator.readthedocs.io/en/latest/readme_link.html}}~\cite{albrecht}.

\begin{table}[ht]
\centering
\begin{tabular}{| c | c | c | c | c | c | c |}
\hline
    \multirow{2}{*}{Algo} & \multirow{2}{*}{$m$} & \multirow{2}{*}{$p$} &   $q$  & $\lambda$ & Am. Time  & Am. Size\\
        &  &  &  (bits) & (bits) & (ms)  & (Bytes)     \\
    \hline
    \hline
    \cite{IZ21} & $28057$ & $167$ & $410$ & $166$ & $5.6$ & $308$\\
    \hline
    \hline
    Ours & $28057$ & $167$ & $300$ & $238$ & $4.8$ ($\boldsymbol{1.2{\times}})$ & $225$ ($\boldsymbol{1.4\times}$) \\
    \hline
    \cite{IZ21} & $17293$ & $131$ & $360$ & \color{red} $106$ & $4.6$ ($\boldsymbol{1.2\times}$) & $270$ ($\boldsymbol{1.1\times}$)\\
    \hline
    Ours & $17293$ & $131$ & $280$ & $152$ & $3.8$ ($\boldsymbol{1.5\times}$) & $210$ ($\boldsymbol{1.5\times}$) \\
    \hline
  \end{tabular}
  \caption{Speed-up of our method compared to \cite{IZ21} when evaluating a coordinate-wise sorting over $4$ vectors of $8$-bit coordinates.
  For each method, the optimum $q$ is reported.
  The amortized (Am.) time and size per coordinate are also shown. We display the amortized time as it allows an absolute comparison, regardless of the dimension of the vectors. The improvement ($\times$) in time and size with respect to the first row is also reported in the respective columns. The red value \textcolor{red}{106} highlights a weak bit security ($\lambda < 128$).
  }
%%  \label{table:comparison-with-IZ}
  \vspace{-5mm}
\end{table}

The first line of the table shows the results of our implementation of \cite{IZ21}'s sorting algorithm using the parameters given in their paper ($m=28057$ and $p=167$, for which $d=9352$ and $\ordp=3$, see Table~3~\cite{IZ21}). 
Using the same parameters $m$ and $p$ (and thus the same $\nslots$ and $\ordp$) but a significantly smaller $B = 7$, the second line shows how our method significantly decreases $q$ thanks to the reduced multiplicative depth of our algorithm. This results in a higher security level $\lambda$ for our solution ($236$ bits) and a 1.2$\times$ gain in computational performance over the other method.

Since our method provides a substantial increase in the security level, in the fourth line we use a lower value for $m$ in order to push the security level down closer to the standard $128$ bits. We take $m\,=\,17293$ and $p\,=\,131$, for which $\nslots=5764$ and $\ordp=3$ (recall \eqref{diag:batching}), thus achieving a security level similar to the one in the first line, and with $B\,=\,7$ we gain a $1.5\times$ speed-up. As an added bonus, the smaller value for $q$ that the flexibility of our method incurs also leads to smaller ciphertexts. Indeed, we show in Table~\ref{table:comparison-with-IZ} that our ciphertexts are $1.5\times$ smaller in size than the ciphertexts in previous works.

The third line shows the results of using the same parameters $m$ and $p$ as in the fourth line but with \cite{IZ21}'s method.
Their resulting security level $\lambda\,=\,106$ dips below the $128$-bit security standard.
\medskip

\textbf{Comparison with non-batched alternatives.}
Up to this point, we have compared the performance of our HTS implementation exclusively to previous best-in-class \emph{batched} implementations of a similar algorithm.
\cite{cong2023efficient} is the state-of-the-art alternative for comparison-based \emph{non-batched} HE algorithms.
Their solution uses the TFHE encryption scheme and improves upon~\cite{CZ22} by designing the fastest homomorphic $k$-nearest neighbors algorithm in the literature.
Extrapolating roughly from the numbers provided in~\cite{cong2023efficient}, we can (generously) estimate the time needed by their algorithm to sort 4 values of 8 bits to be $>0.5$s. Given our results in Table~\ref{table:comparison-with-IZ}, the use of such a method can only be preferable to ours in the pathologically small cases where the ML model only has 90 parameters, which is definitely not representative of present-day deep learning.


